Deterministic and Reliable Software-Defined Vehicles: key building blocks, challenges, and vision

As vehicle systems become increasingly complex, with more features, services, sensors, actuators, and processing units, it is important to view vehicles not just as modes of transportation moving toward full autonomy, but also as adaptive systems that respond to the needs of their occupants. Vehicular services can be developed to support these adaptations. However, the increasing complexity of vehicular service development, even with current standardizations, best practices and guidelines, are insufficient to tackle the high complexity of development, with expectations of up to 1 (U.S.) billion lines of code for a fully (level 5) autonomous vehicle. Within this survey, the paradigm of Deterministic Software Defined Vehicles is explored, aiming to enhance the quality and ease of developing automotive services by focusing on service-oriented architectures, virtualization techniques, and the necessary deterministic intra- and inter-vehicular communications. Considering the main open challenges for such verticals, a vision architecture towards improved services development and orchestration is presented, focusing on: a) a deterministic network configurator; b) a data layer configurator; c) a hypervisor configurator; d) the vehicle abstraction layer; and e) a software orchestrator.

==> sections/section3a.tex <==
The following subsections provide further detail on four most representative data layer solutions in automotive contexts: \ac{mqtt}, \ac{dds}, and \ac{someip} and, more recently, Zenoh. 

%%%%%%%%%%%%%%%%%%%%%%%%
{MQTT}
The \acl{mqtt} protocol was originated in 1999 and is a publish/subscribe protocol. While it is use case agnostic, is mostly associated with lightweight and unreliable communication networks (e.g. \ac{iot} scenarios). It relies on a single point of contact between publishers and subscribers — a broker — and is (usually) based on \ac{tcp} as a transport protocol. \ac{mqtt}, supports basic reliability \ac{qos} configurations and  wild-carding on topic subscription thanks to the existence of a broker. By requiring a centralized point of contact, \ac{mqtt} is known for poor reliability — for its \ac{spof} — and scalability when the number of topics and/or participants scale considerably~\cite{Vector2020}\footnote{Even considering proposed extensions such as \ac{mqtt}-CV to reduce data processed at each subscriber~\cite{Chouali2020}.}.

\begin{figure}[!ht]
	    \centering
	    \includegraphics[width=\columnwidth]{figs/sota/SOTA-MQTT.pdf}
	    \caption[Overview of \acs*{mqtt} functional flow]{Overview of \acs*{mqtt} functional flow~\cite{MQTTmanp69:online}.}
	    \label{fig:sota-mqtt}
	\end{figure}

Even if \ac{mqtt}, through the \ac{mqtt}-\acs*{tsn} alternative, can be agnostic to the transport layer as long as it provides a bidirectional flow~\cite{MQTTSNsp18:online}, it fails to provide and enforce levels and policies of \ac{qos} at several levels — from the topic to the publisher and participant — and in several domains, from reliability to deadline policies, as further detailed in~\cref{fig:sota-dds-qos}.

The effects of having a broker on the message latency are less relevant than the routing or the network load that impact the underlying network layers (remembering that \ac{mqtt} is usually based on \ac{tcp})~\cite{Nenninger2019}. Having a centralized publish/subscriber model, with a single point of contact/broker can support low latencies if the network is properly configured~\cite{Nenninger2019}. However, if needed, a functionally similar solution without broker is possible for example leveraging frameworks such as ZeroMQ\footnote{Available at \myurl{https://zeromq.org/}.}.

%

%%%%%%%%%%%%%%%%%%%%%%%%
{DDS}
The \ac{omg} \acl{dds} is a decentralized alternative. Originated in 2004, can use both unicast or multicast \ac{udp} or \ac{tcp} transport. Like \ac{mqtt}, it follows a publish subscribe paradigm, where participants — that may be both publishers (through \texttt{Data Writers}) or subscribers (through \texttt{Data Readers}) — communicate through topics, as depicted in~\cref{fig:sota-dds}.

While use case agnostic, it is a base for robotic use cases and tools such as \ac{ros}2 and part of \ac{autosar} Adaptive. \ac{dds} is well suited for distributed real-time systems~\cite{Cheikh2010} — for example \ac{dds} and its underlying \ac{rtps} was adapted to embedded FreeRTOS in~\cite{Kampmann2019} and has been proven to be compatible with specific vehicular situations such as handover management~\cite{Cheikh2016}.

\begin{figure}[!ht]
	    \centering
	    \includegraphics[width=\columnwidth]{figs/sota/SOTA-DDS.pdf}
	    \caption[Overview of \acs*{dds} functional flow]{Overview of \acs*{dds} functional flow~\cite{DDS_SPEC}.}
	    \label{fig:sota-dds}
	\end{figure}

%\ac{dds} is a data connectivity standard and middleware set of protocols and \acp{api} that can support a distributed publisher subscriber model. It is a data-centric publish subscribe middleware, \ie the common information between publisher and subscriber is the kind of data exchanged and the exchange of data is via services that publish and subscribe data via topic(s). 

Advantages over \ac{mqtt} include the prioritization of high reliability, availability, redundancy, a complete set of \ac{qos} policies, and automated service discovery~\cite{Kugele2018} within a fully decentralized solution without \acp{spof}. \ac{qos} in this standard is extensively configurable, with reliability, deadline, latency, fault tolerance. and other policies applicable to participants, and topics, as depicted in~\cref{fig:sota-dds-qos}. However, it has a larger memory footprint than \ac{someip} considering its additional \ac{qos} features~\cite{Vector2020}.

Unlike alternatives such as \ac{mqtt}, it does not require a centralized broker, therefore it no longer has a simple point of failure. Other advantages include the dynamic discovery of publishers and subscribers, and the (theoretically) higher performance since it usually considers \ac{udp} as a transport layer and abstracts low level details, while keeping the easy to use, plug-and-play and quality of service capabilities~\cite{WhatisDD6:online}.
\ac{dds} considers messages defined by an Interface Definition Language that are exchanged between \textit{Participants within a Domain} within a \textit{Topic} that is effectively shared across each participant creating a \textit{Global dataspace}.
%. Full decision reliability may then be obtained with sensor fusion, by combining sensory data, where the resulting information is in some sense better than the result of individual sensor~\cite{Elmenreich2007}. This is critical to overcome the limits of certain sensors, e.g., cameras non-line-of-sight (NLOS)~\cite{Anaya2014}.

In addition, \ac{dds} can abstract the transport layer and be interoperable with several alternatives, from inter-process communication (through shared memory), up to \ac{udp} and \ac{tcp} versus the \ac{mqtt} that requires a transport protocol capable of ordered connections (e.g. \ac{tcp})~\cite{MQTTSNsp18:online}. %\ac{dds} 

\begin{figure}[!ht]
	    \centering
	    \includegraphics[width=0.8\columnwidth]{figs/sota/SOTA_DDS_MQTT_QoS.pdf}
	    \caption[\acs*{dds} \acs*{qos} policies vs \acs*{mqtt} 3 levels of \acs*{qos}]{\acs*{dds} \acs*{qos} policies vs \acs*{mqtt} 3 levels of \acs*{qos}. \acs*{dds} policies act at several levels, while \acs*{mqtt} policies only actuate at the number of times each message is delivered (once, at least once or exactly once)~\cite{MQTTmanp69:online,DDS_SPEC}.}
	    \label{fig:sota-dds-qos}
	\end{figure}

Main open challenges on \ac{dds} include~\cite{Koeksal2017}:
\begin{itemize}
	    \item Complexity of the configuration of \ac{dds}: tentatively mitigated by the UML Profile defines a direct mapping between the domain (e.g. automotive) and the \ac{dds} topics, participants, publishers, subscribers and topics~\cite{Tekinerdogan2018}.% and to generate the necessary code from component models.
	    \item Ensuring a predictable scalable performance with the different combinations of \ac{qos} policies and considering that the \ac{dds} entities and endpoints discovery (\ac{dds-sdp}) has issues scaling in function of the number of the nodes. Mitigation techniques include the usage of probabilistic methods based on Bloom filters.
	    \item Integration of \ac{dds} in wired and wireless \acp{wan}: solutions include end-to-end provisioning that relies on controlling the underlying network resources (which opens the possibility of integrating \ac{tsn} configurations within the \ac{dds} usage), the creation of an interconnection services (\ac{dds}-IS), and the abstraction of the end-to-end path (for example through \ac{mpls} tunnels or through the usage of \ac{sip}). 
	    \item Ensuring data consistency within a \ac{dds} context where nodes can fail. A possible mitigation is the introduction of a consensus algorithm to define the value that is supposed to be published on the topic.
	\end{itemize}

The usage of \ac{dds} within the vehicular context is proven to be promising by the works of~\cite{Takrouni2020}. The authors provide a proposal of integration of \ac{dds} as a middleware available to applications by testing a use case with a MATLAB SIMULINK \ac{dds} Blockset developed for the effect. 

The work of~\cite{Kugele2018} tested \ac{dds} (and its open source implementation OpenDDS) for data exchange between vehicular services. The obtained results (\ac{rtt} of packets and time to take-over when a publisher fails) proved the possibility of integration of \ac{dds} in vehicles. %The only added overhead is the middleware, but impact in terms of overall bus load, by removing non subscribed signals that are sent for example, is predictable.

%%%%%%%%%%%%%%%%%%%%%%%%
{SOME/IP}
\ac{someip}\footnote{Available at \myurl{https://some-ip.com/}.} is an automotive service-oriented communication middleware~\cite{Nayak2023} published in 2013. and successfully tested in a vehicular context for example to ensure data exchange between a \ac{adas} and the infotainment of a vehicle~\cite{Kenjic2023}.

It assumes services have methods provided by service instances. These methods can then be invoked by consumer service instances, as depicted in~\cref{fig:sota-someip}. 

\begin{figure}[!ht]
	    \centering
	    \includegraphics[width=\columnwidth]{figs/sota/SOTA-SOMEIP.pdf}
	    \caption[Overview of \acs*{someip} functional flow]{Overview of \acs*{someip} functional flow~\cite{DDS_SPEC}.}
	    \label{fig:sota-someip}
	\end{figure}

As a middleware, it includes support not only for the publish and subscription of information but also the discovery of services, serialization of data and \ac{rpc}. It includes a service discovery concept, with messages for finding, offering and subscribing services between a client and a server. Unlike \ac{dds}, it does not support \ac{qos}~\cite{Bhat2020}, which is solved at the application level~\cite{Vector2020}. \ac{someip} leverages  \ac{ip} and Ethernet as a \ac{mac} layer for service-oriented communication within vehicles. 

It includes a non-static service discovery protocol that is based on both uni- and multi-cast. This protocol adds overhead in the overall setup time (\ie the time until a subscription of a service can start)~\cite{Cheikh2010}. According to~\cite{Cheikh2010}, such times can greatly vary depending on the configurations on the phases time\footnote{Services in \ac{someip} can be in three phases: an initial wait phase, a repetition phase, and a main phase. The wait phase timing configuration, in which the service ignores any subscription request, is of particular importance to ensure the minimization of these times.}.

The main advantages of \ac{someip} include its design as a middleware compatible with the existing vehicular stacks, namely \ac{autosar} based \acp{ecu}~\cite{Wagner2016,Kyung2023} — in fact, the Adaptive platform leverages this middleware for message control to support high performance computing within the vehicle, dynamic linking of services and clients during runtime in a \ac{soa} fashion ~\cite{Bhat2020}. It can also support security extensions~\cite{Gehrmann2020}, ensuring is secure for vehicular contexts with authentication and confidentiality of data~\cite{Khemissa2023}.

\ac{someip} main disadvantage is its total reliance on \ac{ip} and not supporting existing vehicular buses such as \ac{can}. The work in~\cite{Gopu2016} proposes an adaptation to the \ac{can} bus that, unlike the standard, supports non-static configuration of nodes' identifiers within the network via a find/offer pattern Service Discovery~\cite{Casparsen2022}. %; a publish/subscribe pattern to exchange data; and a request response for \ac{rpc}. The middleware should not be Pub/Sub only. It should support request-response for \ac{rpc} scenarios.  

Security is one of the main challenges in the migration within \ac{someip}, with issues relating to impersonation attacks that change values within a service, session stealing or \ac{dos} attacks based on chaining \ac{ttl} fields in messages of the discovery process.

%\ac{someip} can benefit from hardware (\ac{fpga}) accelerated tasks, such as serialization~\cite{Elbahnihy2020}.

%One of the main gaps of \ac{autosar} is the management of faults in \acp{ecu} or services.~\cite{Bhat2020} proposes a fault tolerance solution leveraging the \ac{someip} middleware. 

%%%%%%%%%%%%%%%%%%%%%%%%
{Zenoh}
Eclipse Zenoh\footnote{Available at \myurl{https://zenoh.io/}.} is another publish/subscribe middleware alternative, with most usages being related to autonomous vehicles and robotics \cite{Deployme63:online}. 

Like \ac{dds}, it is a decentralized solution with dynamic discovery of other nodes. However, it can be configured to support several degrees of centralization, as depicted in~\cref{fig:background-zenoh}, which range from completely peer-to-peer (in both clique and mesh topologies) up to a centralized version based on the existence of routers, that route data between clients and local subnets of peers. Zenoh applications in peer mode run discovery protocols (through multicast and gossip scouting) to discover other applications or Zenoh routers~\cite{Deployme63:online}.

\begin{figure}
	    \centering
	    \includegraphics[width=1\columnwidth]{figs/sota/SOTA-Zenoh-Modes.pdf}
	    \caption[Zenoh deployment modes]{Zenoh deployment modes \cite{Deployme63:online}.}
	    \label{fig:background-zenoh}
	\end{figure}

Zenoh, like \ac{dds}, support different transport protocols to be used between Zenoh peers, such as \ac{tcp}, \ac{udp}, and Unix sockets, but also QUIC and web sockets~\cite{liang2023performance}. Also like \ac{dds} and \ac{mqtt}, Zenoh supports \ac{qos} through multiple levels of reliability or fragmentation \cite{Deployme63:online}.

However, Zenoh distinguishes itself from previous solutions for providing built-in support for storing data with sharding and replication, as well as providing support for querying and aggregating that data \cite{Deployme63:online}.

%%%%%%%%%%%%%%%%%%%%%%%%
{Other alternatives}
\ac{coap} is a request/response interaction model with discovery of services of resources and can be used for \ac{m2m} communication between constrained nodes and networks~\cite{rfc7252}. The work of~\cite{Laaroussi2018} proves the overall advantage of \ac{coap} in terms of end to end latency and throughput.

\ac{http} is a well-known alternative, but like \ac{coap} is request/response and is therefore not suited for critical vehicular scenarios where the decoupling of the producer of the information from the consumer(s) is critical to ensure reliability. 

The oneM2M set of standards is aimed to \ac{m2m} \ac{iot} scenarios, with (planed) support for interoperability with \ac{http}, \ac{coap}, \ac{mqtt}, \ac{3gpp} and offering vehicular centric features (including support of mobility of the vehicular nodes and required low latency), service discovery and device management\footnote{Specification at \myurl{https://onem2m.org/technical/published-specifications}.}.

A middleware for dynamic configuration of \ac{qos} is proposed by~\cite{Ouedraogo2018} with a data layer agnostic protocol (with support \ac{http}, \ac{coap}, \ac{mqtt}, oneM2M) is used enforce \ac{qos} policies. The authors emphasize the need for \ac{qos} modules to be protocol agnostic as  much as possible, while being flexible to support multiple \ac{qos} metrics in a online manner.


==> vars/packagesIEEE.tex <==
\usepackage{amsmath,amssymb,amsfonts}
%\usepackage[backend=biber, doi=true, url=true, style=ieee]{biblatex}
\usepackage{algorithmic}
\usepackage[pdftex]{graphicx}
\usepackage{tikz}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{subcaption}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{multicol}
\usepackage{siunitx}
%\usepackage{acro}[=v2]
\usepackage{colortbl}

\usepackage[nolist]{acronym} % For acronyms
\usepackage{verbatim}
\usepackage{float}
\usepackage{hyperref}
\usepackage{cleveref}
%\usepackage{multirow}
%\usepackage[ruled,noend]{algorithm2e}
%\SetAlFnt{\small}
%\SetKwComment{Comment}{$\triangleright$\ }{}
\usepackage{nicefrac}
\usepackage{tablefootnote}
%\usepackage{fancyhdr} % to change headers and footers
%\usepackage{algorithm}
%\usepackage{algpseudocode}
%\usepackage{todonotes}
\usepackage{booktabs}
\usepackage[super]{nth}
\usepackage{etoolbox}
\usepackage{threeparttable}
\usepackage{listings}
\usepackage{pgfplots}
\usepackage{tabularx}
%\usepackage{svg}
%\usepackage[finalizecache,cachedir=.]{minted}
%\usepackage[frozencache,cachedir=.]{minted}
%\setminted{fontsize=\small}
%\fvset{fontsize=\footnotesize} % Make Code blocks smaller than text
\usepackage{csquotes}
\usepackage{multirow} 


==> vars/table-arch-servicedescriptor.tex <==
\begin{table}[!ht]
    \caption[Service descriptor proposal with main fields and their types]{Service descriptor proposal with main fields and their types.}
    \label{fig:arch-serviceDescriptor}
    \centering
    \begin{tabular}{lp{0.1\columnwidth}p{0.4\columnwidth}} \hline 
         \textbf{Value}&  \textbf{Type of value}& \textbf{Unit}\\ \hline 
          
         Bandwidth & Numeric & \si{\bit\per\second} \\ \hline 
         Latency   & Numeric & \si{\milli\second} \\ \hline 
         \acs*{cpu} & Numeric & Virtual \acsp*{cpu} \\ \hline 
         Deadline & Numeric & \si{\milli\second} \\ \hline 
         Period & Numeric & \si{\milli\second} \\ \hline 
         Durability & Numeric & \si{\milli\second} \\ \hline 
         Delivery & Enum & Exactly once, at least once, more than once \\ \hline 
         Memory & Numeric & \si{\mega\byte} \\ \hline 
         Storage & Numeric & \si{\byte} \\ \hline 
         GPU & Boolean, Numeric & Requires or not, VRAM \\ \hline 
         Replicas & Numeric & Expected minimum of replicas \\ \hline 
         Wired & Boolean & Yes/no (wireless communications) \\ \hline 
         Location & Enum & Within the vehicle front left, front right, center, back left, back right \\ \hline 
         Federation & Enum & Edge, cloud, both \\ \hline 
         Safety Service & Boolean & Yes/no \\ \hline 
         Service Type & Enum & Docker, Kubernetes, Script \\ \hline 
         Service Name & String & Friendly name \\ \hline 
 \end{tabular}

\end{table}

% \begin{figure}[!ht]
%     \centering
%     %\includegraphics[width=0.6\linewidth]{figs/arch/Arch-ServiceDescriptor.pdf}
%     \includesvg[width=0.6\linewidth]{figs/arch/Arch-ServiceDescriptor.svg}
    
    
% \end{figure}

==> vars/table-sota-ethernet.tex <==
\begin{table}[!ht]
\centering
\caption[Comparison of main Ethernet alternatives]{Comparison of main Ethernet alternatives~\cite{MindtheG86:online}.}
\label{tab:background_Ethernet-Evolution}
\resizebox{\columnwidth}{!}{%
%\begin{tabular}{p{0.20\columnwidth}p{0.15\linewidth}p{0.20\columnwidth}p{0.15\columnwidth}p{0.15\columnwidth}p{0.15\columnwidth}}
	\begin{threeparttable}[t]
		\begin{tabularx}{\columnwidth}{XXXX}
		\hline
				\textbf{Name} 		    & \textbf{Standard}					   & \textbf{Bandwidth} 	& \textbf{Cabling}  \\ \hline
				10BASE-T1S & IEEE 802.3cg  & \qty{10}{\mega\byte\per\second} & Single balanced twisted-pair copper \\ \hline
				100BASE-T1 & IEEE 802.3bw & \qty{100}{\mega\byte\per\second} & Single balanced twisted-pair copper \\ \hline
				1000BASE-T1 & IEEE 802.3bp & \qty{1000}{\mega\byte\per\second} & Single balanced twisted-pair copper \\ \hline
				1000BASE-RHC & IEEE 802.3bv & \qty{1000}{\mega\byte\per\second} & Step index plastic optical fiber \\ \hline
				2.5G, 5G, 10G BASE-T1 & IEEE 802.3ch &  2.5, 5, \qty{10}{\giga\byte\per\second} & Single balanced pair of conductors \\ \hline
				2.5, 5G, 10G, 25G, 50G BASE-AU & IEEE STD 802.3CZ-2023 & 2.5, 5, 10, 25, \qty{50}{\giga\byte\per\second} & IEC 60793-2-10 Type A1a.2 (OM3) glass multi-mode optical fiber \\ \hline
				25GBASE-T1 & IEEE P820.3cy\tnote{a} & \qty{25}{\giga\byte\per\second} & Single balanced pair of conductors \\ \hline
				Multi-Gig Automotive Ethernet~\cite{ASHJAEI2021102137} & IEEE 802.3ch-2020 & 2.5, 5, \qty{10}{\giga\byte\per\second} & Single balanced pair of conductors  \\ \hline
				The Future\tnote{b} & IEEE 802.3df & 800 Gb/s & Single x8 copper or optical \\ \hline
			\end{tabularx}
		 
		 	\begin{tablenotes}
			 	\item[a] Future standard.
			 	\item[b] As described in \myurl{https://standards.ieee.org/beyond-standards/ethernets-next-bar/}.
		 	\end{tablenotes}
 	\end{threeparttable}%
}
\end{table}
